Security policies for distributed systems

A security policy specifies a security property as the maximal information flow. A distributed system composed of interacting processes implicitly defines an intransitive security policy by repudiating direct information flow between processes that do not exchange messages directly. We show that implicitly defined security policies in distributed systems are enforced, provided that processes run in separation, and possible process communication on a technical platform is restricted to specified message paths of the system. Furthermore, we propose to further restrict the allowable information flow by adding filter functions for controlling which messages may be transmitted between processes, and we prove that locally checking filter functions is sufficient for ensuring global security policies. Altogether, global intransitive security policies are established by means of local verification conditions for the (trusted) processes of the distributed system. Moreover, security policies may be implemented securely on distributed integration platforms which ensure partitioning. We illustrate our results with a smart grid case study, where we use CTL model checking for discharging local verification conditions for each process under consideration.

==> figs/building_fta.tex <==
\[\begin{array}[]{|c|c|c|c|}
  \hline
  \alpha  & \fta_{\mbox{Red}}(\alpha) & \fta_{\mbox{Bypass}}(\alpha) & \fta_{\mbox{Crypto}}(\alpha)  \\
  \hline
  \fB    &   \fB & & \\
  \fB

\end{array}\]


==> figs/flow_intro.tex <==
\begin{tikzpicture}
  \node[draw,inner sep=3pt] (p1) {$\pi_1$} ;
  \node[draw,inner sep=3pt,anchor=west] at ($(p1.east) + (0.4,0)$) (p2) {$\pi_2$} edge[pre] (p1) ;
  \node[draw,inner sep=3pt,anchor=west] at ($(p2.east) + (0.4,0)$) (p3) {$\pi_3$} edge[pre] (p2) ;
\end{tikzpicture}


==> figs/tikzstyles.tex <==

\tikzstyle{place}+=[inner sep=0,minimum size=3mm]
\tikzstyle{transition}+=[fill,minimum width=3mm,minimum height=0.5mm,font=\tiny]
\tikzstyle{synchron}=[fill,inner sep=0,minimum size=1.4mm,circle]
\tikzstyle{observ}=[draw,fill=white,line width=1pt,inner sep=0,minimum size=1.4mm,circle]
\tikzstyle{triggert}=[draw,fill,regular polygon,regular polygon sides=3,inner
     sep=0pt,minimum size=1.7mm,yshift=0.5mm]
\tikzstyle{triggerb}=[draw,fill,regular polygon,regular polygon sides=3,inner
     sep=0pt,minimum size=1.7mm,rotate=180,yshift=0.5mm]
\tikzstyle{triggerl}=[draw,fill,regular polygon,regular polygon sides=3,inner
     sep=0pt,minimum size=1.7mm,rotate=90,yshift=0.5mm]
\tikzstyle{triggerr}=[draw,fill,regular polygon,regular polygon sides=3,inner
     sep=0pt,minimum size=1.7mm,rotate=270,yshift=0.5mm]
\tikzstyle{component}=[fill=yellow!30,draw=orange,thick]
\tikzstyle{engine}=[fill=yellow!30,draw=orange,thick]
\tikzstyle{func}=[fill=gray!60,inner sep=0pt]
\tikzstyle{offer}=[thick,red]
\tikzstyle{notif}=[thick,black!70]
%\tikzstyle{initial}=[after node path={(\tikzlastnode.235) edge[pre] ++(235:0.3)}]
\tikzstyle{initial}=[after node path={(\tikzlastnode.225) edge[pre] ++(225:0.3)}]
\tikzstyle{initialUp}=[after node path={(\tikzlastnode.135) edge[pre] ++(135:0.3)}]
\tikzstyle{transitionh}=[transition,fill=black,minimum height=0.5mm,minimum width=3mm]
\tikzstyle{transitionv}=[transition,fill=black,minimum height=3mm,minimum width=0.5mm]
\newcommand{\colo}[1]{ \begin{array}{l} #1 \end{array}}
\newcommand{\coloc}[1]{ \begin{array}{c} #1 \end{array}}
\newcommand{\colod}[1]{ \begin{array}{r} #1 \end{array}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\off}{\mathit{off}}
\newcommand{\clks}{\mathrm{C}}

